US Cosmic Visions: New Ideas in Dark Matter 2017: Community Report

This white paper summarizes the workshop "U.S. Cosmic Visions: New Ideas in Dark Matter" held at University of Maryland on March 23-25, 2017.

==> acknowledgments.tex <==
\section*{Acknowledgements}


==> wg-targets.tex <==
This report surveys two broad possibilities for the nature of DM and its interactions, the specific milestones they suggest, and the opportunities presented by  small experiments to make important progress in exploring these possibilities.

One of the goals of the ``New Ideas in Dark Matter" workshop was to identify well motivated areas of dark matter parameter space, and assess how small experiments can explore these regions.  To this end, each Working Group was tasked with identifying exciting science opportunities; these were summarized in the workshop close-outs.  The opportunities identified by each working group are summarized below:

\subsubsection{WG1}

Direct-detection experiments play a unique and essential role in our quest to identify the DM.  Several proposals and ideas exist for new experiments that present a low-cost opportunity --- well within the ``small-project'' scale --- to probe DM with masses between the meV to GeV scale, many orders of magnitude in mass below the planned searches by the G2 experiments LZ and SuperCDMS.  In fact, the working group recognizes that recent advances in theory and experiment means that {\it now} is the right time for targeted investments to bring to fruition several recent new ideas and proposals and develop them into real experiments.  

Several well-motivated DM candidates can be probed.  This includes DM that obtains its relic abundance from thermal freeze-out, from an initial asymmetry between DM particles and anti-particles, from freeze-in, through $3\to 2$ annihilations in models of Strongly Interacting Massive Particles (SIMPs), from its elastic scattering off Standard Model particles in the ``Elastically Decoupling Relics'' (ELDERs) scenario, or from the misalignment mechanism.  In several cases, {\it sharp theory targets} in parameter spaces can be identified, which can be probed by first-generation, low-cost experiments with target exposures of as little as 100 gram-days. 

Direct detection also provides the {\it only} possibility to test several freeze-in scenarios: in these scenarios, DM is never in thermal equilibrium with ordinary matter in the early Universe --- necessitating tiny interactions between DM and Standard Model particles --- but a small residual annihilation of Standard Model to DM particles through an ultralight mediator allows the correct relic abundance to be obtained.  Although the couplings are small, the ultralight mediator leads to an enhancement of the direct-detection cross section at low momentum transfers, allowing this scenario to be probed with new direct-detection experiments but not with other experiments.  
We emphasize that the {\it same} experiment can probe {\it many} DM candidates.  At the same time, there is a need for experiments that probe DM couplings to electrons as well as experiments that probe DM couplings to nuclei.  

A discovery of a new particle at an underground direct-detection experiment would constitute strong evidence that such a particle constitutes all or at least part of the DM.  
%This is in contrast to accelerator-based probes, where a discovery of a new particle, while profound, would only require that the particle's lifetime is larger than a fraction of a second in order to escape the detector unseen.  
This emphasizes that a small-scale program will be most successful if it contains a multitude of approaches to probe DM.  

%%A key point emphasized by the working group is that by leveraging new theoretical ideas together with technological advances that allow for the detection of low-threshold signals, vast regions of DM parameter space can be explored by small detectors that are only a fraction of the cost of the G2 experiments.  
%%The close collaboration between theorists and experimentalists has been essential in developing these new ideas, which are now ripe for implementation.  

\subsubsection{WG2}
In the case of ultra-light bosonic dark matter, the QCD axion remains one of the best motivated dark matter candidates.  While axions provide perhaps the simplest solution to the strong-CP problem, these models also inevitably produce dark matter via release of their initial potential energy density.   Axion dark matter searches and cosmic microwave background experiments provide complementary probes of inflation;  a measurement of the axion mass by detection of the dark matter beam would also immediately determine or constrain the energy scale of cosmic inflation;  Recent phenomenology has also indicated a possibly rich interplay between QCD axions and the electroweak hierarchy problem.

Searches for the QCD axion, including continuation of the current ADMX generation 2 experiment should be highly prioritized in any future dark matter program.  However it should be noted that similarly cost-effective experimental techniques have been identified that would cover a broad range of masses for well-motivated and more general scalar, pseudoscalar, or vector dark matter models.  These experiments would import non-traditional detector technology that has nonetheless been well developed in other fields of physics – atom interferometry, nuclear magnetic resonance, fifth force measurements.  Large improvements sensitivity to low mass bosonic dark matter can and should be quickly obtained by engaging these other communities in cross-disciplinary collaborations.  

\subsubsection{WG3}

The next generation of small-scale accelerator experiments offer an opportunity for the US DM program to play {\it the} leading role in light DM and dark sector physics over the next decade. Accelerator experiments have become essential tools in probing DM in the vicinity of known Standard Model mass scales, roughly MeV - TeV.  A thermal origin is a well-motivated paradigm that has received much attention during the last decades, and it provides sharp theoretical guidance for new experimental probes. Among the new DM parameter space highlighted in this report, sub-GeV hidden sector thermal DM that can annihilate directly into Standard Model final states stands out both for its predictiveness and testability in laboratory experiments. Accelerators can cover {\bf all} of the direct annihilation thermal targets as well as much of the natural parameter space for the secluded annihilation DM scenario.

New precision fixed-target and collider experiments are uniquely capable of decisively testing this possibility, 
benefiting from the fact that the rate of relativistic DM production at accelerators is predicted from thermal freeze-out, 
whereas the rate of non-relativistic DM scattering is highly sensitive to the details of the dark sector particles.

The discussion in this section is focused on sub-GeV directly annihilating thermal DM, because of the dramatic scientific impact of reaching this milestone as well as the opportunity to do so timely.  At the same time, we emphasize that the reach of an accelerator-based program is broad.  
The proposed experiments will explore a wide parameter space for secluded thermal DM, despite the absence of a sharp sensitivity milestone for this scenario, as well as models of DM with a quasi-thermal origin such as asymmetric DM and the SIMP/ELDER scenarios.  

Finally, a key feature of the next generation accelerator program highlighted in this working group is that the various experimental methods we survey leverage proven techniques and existing technology, thus enabling the deployment of the majority of the proposals in the very near future.
\subsubsection{WG4}

The hunt for dark matter now crosses multiple frontiers and benefits from vibrant communication between many subdisciplines of physics, including astrophysics, cosmology, and nuclear, atomic, and condensed matter physics.  Innovations springing from these collaborations have created a wealth of new ideas that can be explored by inexpensive experiments.  In addition, there are various existing experimental anomalies that may be pointing towards dark sector physics.  We highlight a few areas where research support is particularly timely and will lead to great improvements in our understanding of dark matter and the dark sector.

\begin{itemize}

\item {\em Importance of Investment in Theory.} Healthy support for theory is essential to maintaining the flow of creative and cross-disciplinary ideas that have been seen in recent years, and which may finally unmask the particle identity of dark matter.

\item {\em Nuclear and Accelerator Tests of the $^8$Be Anomaly.}  The $^8$Be anomaly strongly motivates proposed followup nuclear experiments that are fast (under 2 years) and cheap (a small fraction of the small projects threshold), as well as isotope shift spectroscopy experiments and accelerator searches for new bosons with masses $\sim 10$ MeV and electron couplings $\varepsilon \sim 10^{-4} - 10^{-3}$.

\item {\em Synergy with Cosmology and Astrophysics.}  Small investments in simulations and astroparticle theory can leverage the enormous amount of cosmological data already being collected and are certain to provide not just {\em constraints} on dark matter {\em candidates}, but {\em measurements} of the properties of {\em dark matter}.

\item {\em Prominence of the 1 to 100 MeV Mass Scale.}  New models, astrophysical observations, and existing experimental anomalies point to the 1 to 100 MeV mass scale as a high-value target region for dark matter and dark mediator searches.

\item {\em Microlensing Searches for Solar Mass Black Hole Dark Matter.}  The LIGO discovery of gravitational waves from colliding black holes strongly motivate a proposed microlensing search that can confirm or exclude the possibility of intermediate mass black hole dark matter using existing facilities with minimal funding.

\end{itemize}


